Gaia Data Release 2: first stellar parameters from Apsis

The second Gaia data release (Gaia-DR2) contains, beyond the astrometry, three-band photometry for 1.38 billion sources. We have used these three broad bands to infer stellar effective temperatures, Teff, for all sources brighter than G=17 mag with Teff in the range 3000-10 000 K (161 million sources). Using in addition the parallaxes, we infer the line-of-sight extinction, A_G, and the reddening, E[BP-RP], for 88 million sources. Together with a bolometric correction we derive luminosity and radius for 77 million sources. These quantities as well as their estimated uncertainties are part of Gaia-DR2. Here we describe the procedures by which these quantities were obtained, including the underlying assumptions, comparison with literature estimates, and the limitations of our results. Typical accuracies are of order 324 K (Teff), 0.46 mag (A_G), 0.23 mag (E[BP-RP]), 15% (luminosity), and 10% (radius). Being based on only a small number of observable quantities and limited training data, our results are necessarily subject to some extreme assumptions that can lead to strong systematics in some cases (not included in the aforementioned accuracy estimates). One aspect is the non-negativity contraint of our estimates, in particular extinction. Yet in several regions of parameter space our results show very good performance, for example for red clump stars and solar analogues. Large uncertainties render the extinctions less useful at the individual star level, but they show good performance for ensemble estimates. We identify regimes in which our parameters should and should not be used and we define a "clean" sample. Despite the limitations, this is the largest catalogue of uniformly-inferred stellar parameters to date. More precise and detailed astrophysical parameters based on the full BP/RP spectrophotometry are planned as part of the third Gaia data release.

==> tex/_region_.tex <==
\message{ !name(cluster-ag-estimation.tex)}
\message{ !name(cluster-ag-estimation.tex) !offset(-2) }
\section{Estimation of cluster extinction}
\label{appendix:mean-cluster-extinction}

As our extinction and reddening estimates are very noisy and also constrained to be non-negative, their combination (for parameter estimation) becomes non-trivial. Here we first outline how to use our results, using the example of estimating the extinction in a star cluster. Second, we show that the sample mean is generally a poor estimator that suffers from strong biases. Third, we use the clusters to obtain another global uncertainty estimate for our extinctions (independent of section~\ref{ssec:extinction-in-halo}).

Suppose we have estimated \ag\ for $N$ cluster members, whereby each estimate has a common uncertainty $\sigma$. (We will not use out inferred confidence interval -- 16th and 84th percentiles -- for each extinction.) 
Suppose further that the intrinsic scatter in the true extinctions is negligible compared to this uncertainty.\footnote{This is only true for low-extinction clusters.  Taking all PARSEC models with $\Zabun=\Zabun_\odot=0.0152$, $\a0=2$\,mag and $\log_{10}$($age$/yr)=9.7, then \ag\ ranges from 1.10 to 1.68\,mag and \ebpminrp\ ranges from 0.73 to 0.84\,mag.}  
Then the true (but unknown) extinctions are all equal to the cluster extinction, $\mu$.  We want to infer $\mu$ and $\sigma$ from the $N$ measurements. 
The likelihood $P(\ag|\mu,\sigma)$ which makes the fewest assumptions in this case is the Gaussian. If $\ag$ is additionally restricted to a finite range (as is the case for our \extratrees outputs), then the least-informative likelihood distribution is a Gaussian truncated over this range \citep{Dowson1973}.\footnote{The least-informative distribution is derived from a maximum entropy argument, as used in section~\ref{ssec:extinction-in-halo} to arrive at the exponential distribution for high Galactic latitudes.
The maximum entropy distribution is different in the present case because we now impose a mean $\mu$ and a
variance $\sigma^2$, which are the parameters of our model we want to find.}
This we can write (properly normalized) as
%{\modi Therefore the likelihood takes the form of a Gaussian, to first order.  However, we also must account for the restricted range of AG predictions (see sect. 3.3), which leads us to adopt a truncated Gaussian likelihood function\footnote{In absence of further knowledge, the distribution with the largest entropy should be chosen as the least-informative default, which according to, the maximum entropy distribution for given first and second moments for a real-valued random variable $x$ restricted to some finite interval $x\in[a,b]$ is a truncated Gaussian over that interval. It is no longer an exponential as in section~\ref{ssec:extinction-in-halo}, because we now impose a mean $\mu$ and a variance $\sigma^2$, which are the parameters of our model we want to find.} for a single star}
\begin{equation}\label{eq:single-star-likelihood-cluster-ag}
p(\ag|\mu,\sigma)=
\left\{
\begin{array}{ll}
\frac{\frac{1}{\sigma\sqrt{2\pi}}\exp\left[-\frac{1}{2}\left(\frac{\ag-\mu}{\sigma}\right)^2\right]}{\frac{1}{2}\left[
{\rm erf}\left(\frac{\ag^{\rm max}-\mu}{\sqrt{2}\sigma}\right)
+{\rm erf}\left(\frac{\mu-\ag^{\rm min}}{\sqrt{2}\sigma}\right)
\right]}
& \textrm{for} \ \ag\in[\ag^{\rm min}, \ag^{\rm max}] \\
\\
0 & \textrm{otherwise}
\end{array}
\right.
\,\textrm{,}
\end{equation}
%
where
%$\mu$ is the mode of the distribution -- provided it lies within $[\ag^{\rm min}, \ag^{\rm max}]$  -- and we use the definition
%
\begin{equation}
{\rm erf}(z)=\frac{2}{\sqrt{\pi}}\int_0^z e^{-t^2}dt
\,\textrm{.}
\end{equation}
Throughout this appendix we fix $\ag^{\rm min}=0$ and $\ag^{\rm
max}=3.609$\,mag, which is the \ag\ range in the \priam training sample
($\a0\in[0,4]$\,mag).\footnote{Since no cluster can have negative intrinsic extinction, we can guarantee that $\mu\geq\ag^{\rm min}=0$. However, for extremely extincted clusters it may happen that $\mu\geq\ag^{\rm max}=3.609$\,mag, i.e., the mode may not be inside our parameter range.}

For the set of $N$ cluster members, the total likelihood is just the product of the single-star likelihoods. Note that due to the limitation $\ag\in[0,3.609]$ the normalisation constant of the likelihood now depends on the cluster extinction $\mu$ (and not only on $\sigma$). For this reason, there is no analytic solution for either of the parameters.
In particular, the sample mean is no longer a useful estimator for the cluster extinction $\mu$, which is the mode (and not the mean) of the truncated Gaussian
(provided it lies within $[\ag^{\rm min}, \ag^{\rm max}]$). We illustrate this with a simulation in which we draw a number of samples from a truncated Gaussian with specified true extinction $\mu$ and fixed $\sigma=0.46$\,mag and compare the sample mean, $\langle\ag\rangle$, to the true extinction of the simulation. As is obvious from Fig.~\ref{fig:gspphot-cluster-bias-sample-mean-demo}, if the true extinction approaches the lower or upper limit, the sample mean becomes biased. Only for clusters with intrinsic extinctions between about 1.3\,mag and 2.4\,mag can we expect the sample mean to be a reliable estimator, i.e.\ when the intrinsic extinction is about $3\sigma$ or more away from the lower and upper limits. For low-extinction clusters, the bias of the sample mean will be largest and of the same order as $\sigma$ for our \ag\ estimates, i.e.\ we may obtain a 0.4\,mag or larger sample mean $\langle\ag\rangle$ for clusters whose expected intrinsic extinction is zero. We emphasise that this bias does \textit{not} diminish if we have more cluster members, as is also clear from Fig.~\ref{fig:gspphot-cluster-bias-sample-mean-demo}.

\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{figures/gspphot-cluster-bias-sample-mean-demo.pdf}
\caption{Simulation showing how the sample mean is a biased estimator using of the cluster extinction using 100 cluster member stars (red) and 2000 members (blue) with $\sigma=0.46$\,mag. Shaded areas show the central 68\% confidence interval estimated from 101 simulations.}
\label{fig:gspphot-cluster-bias-sample-mean-demo}
\end{center}
\end{figure}

\begin{figure*}
\begin{center}
\includegraphics[width=0.95\textwidth]{figures/gspphot-cluster-extinction-estimation.pdf}
\caption{Estimating cluster extinctions for Pleiades (a,e), Praesepe (b,f), Hyades (c,g) and NGC884 (d,h).
%
The top row shows likelihood maps of cluster extinction $\mu$ and global uncertainty estimate $\sigma$.
Contours show 68\%, 90\%, 95\% and 99\% confidence regions. Horizontal dashed lines indicate our global uncertainty estimate of 0.46\,mag from section~\ref{ssec:extinction-in-halo}. Vertical dashed lines are $\ag\sim(0.6-1.0)\cdot\a0$
\citep[][Fig.~17 therein]{2010A&A...523A..48J} for literature estimates of  
$\a0\sim 3.1\cdot E(B-V)$ from \citet{2003A&A...397..191P}.
%
The bottom row shows, for each cluster, the histogram of estimated \ag\ (black) and the maximum-likelihood estimate of the truncated Gaussian (red).
}
\label{fig:gspphot-cluster-extinction-estimation}
\end{center}
\end{figure*}

Since the sample mean is no longer a useful estimator in general, we must use the likelihood from equation~\ref{eq:single-star-likelihood-cluster-ag} in order to estimate parameters.
We find the maximum of the likelihood (Bayesians may add priors). In Table~\ref{table:cluster-extinction-estimates} we provide our estimates for the 46 clusters from  \citet{DR2-DPACP-31} and Fig.~\ref{fig:gspphot-cluster-extinction-estimation} shows the likelihood function over $\mu$ and $\sigma$ for the Pleiades, Praesepe, Hyades and NGC884. For Praesepe and the Pleiades, the estimated cluster extinctions agree very well with the literature values. Emphasizing the point from Fig.~\ref{fig:gspphot-cluster-bias-sample-mean-demo}, the sample mean extinction for Praesepe is $\langle\ag\rangle=0.4$\,mag, whereas the maximum likelihood estimate is actually $\hat{\mu}=0$\,mag (see Table~\ref{table:cluster-extinction-estimates}), which compares 
favourably with the literature estimate of 0.03\,mag used in section \ref{sec:dust_clusters}. For the Pleiades, the sample mean is 0.48\,mag while the maximum likelihood estimate is only 0.11\,mag (cf.\ literature estimate of 0.124\,mag). We obtain $\hat\sigma= 0.59$\,mag and 0.55\,mag for Praesepe and Pleiades, respectively, which are larger than our global uncertainty estimate of 0.46\,mag from section~\ref{ssec:extinction-in-halo}. In the case of the Hyades we clearly overestimate the cluster extinction with $\hat{\mu}=0.209$\,mag while $\hat\sigma=0.42$\,mag is slightly below our global uncertainty estimate. (Note from Fig.~\ref{fig:gspphot-cluster-extinction-estimation} that these two quantities are negatively correlated when approaching the lower boundary.) Given that we only have 369 Hyades members with \ag\ estimates, we suspect this to be ``shot noise''. Indeed, simulating 100 Hyades-like samples, each with true $\mu=0.01$\,mag, true $\sigma=0.46$\,mag, and 369 stars, we observe similar bad misestimations in 8\% of the cases. It may come as a surprise that 369 stars is not necessarily sufficient to reliably estimate the cluster extinction and the scatter. The explanation is that for a low-extinction cluster such as the Hyades, the truncation of the Gaussian is dominant: we are trying to infer a pathological distribution. In such a case, estimating the cluster extinction $\mu$, which is the mode of the distribution, requires an estimate of the full density distribution (as opposed to a ``point estimate'' such as the sample mean). As an example of a cluster with higher extinction, the maximum-likelihood estimate of NGC884 also agrees well with literature results. Nevertheless, although our maximum-likelihood estimates of the cluster extinctions are largely consistent with the expected values, the random errors are still far too large for detailed studies of Hertzsprung-Russell diagrams in clusters. 

\begin{table}
\caption{Estimates of the cluster extinction using the
sample mean $\langle\ag\rangle$ (which is biased) and the maximum likelihood (ML) estimates of $\mu$, as well as the global uncertainty $\sigma$.
Clusters are sorted with descending number of member stars. Nearby clusters within 250pc are marked in bold face.
Cluster memberships are taken from \citet{DR2-DPACP-31}.}
\label{table:cluster-extinction-estimates}
\begin{center}
\begin{tabular}{lrrrr}
\hline
      & no.\ of & & \multicolumn{2}{c}{ML estimates} \\
name & stars & $\langle\ag\rangle$  & $\hat{\mu}$ & $\hat{\sigma}$ \\
 &  & mag & mag & mag \\
\hline
%
NGC3532 & 1217 & 0.293 & $0.000^{+0.005}_{-0.000}$ & $0.406^{+0.007}_{-0.009}$ \\
NGC2437 & 962 & 0.538 & $0.503^{+0.012}_{-0.013}$ & $0.309^{+0.011}_{-0.008}$ \\
NGC2516 & 894 & 0.373 & $0.083^{+0.042}_{-0.052}$ & $0.427^{+0.025}_{-0.020}$ \\
NGC2682 & 724 & 0.371 & $0.000^{+0.025}_{-0.000}$ & $0.479^{+0.008}_{-0.020}$ \\
\textbf{Pleiades} & 721 & 0.478 & $0.113^{+0.056}_{-0.073}$ & $0.544^{+0.034}_{-0.027}$ \\
NGC2168 & 709 & 0.629 & $0.619^{+0.010}_{-0.012}$ & $0.283^{+0.009}_{-0.008}$ \\
NGC6475 & 612 & 0.373 & $0.165^{+0.042}_{-0.055}$ & $0.381^{+0.031}_{-0.020}$ \\
\textbf{Praesepe} & 485 & 0.464 & $0.000^{+0.078}_{-0.000}$ & $0.585^{+0.005}_{-0.047}$ \\
IC4651 & 474 & 0.506 & $0.360^{+0.037}_{-0.047}$ & $0.423^{+0.031}_{-0.022}$ \\
NGC0188 & 450 & 0.585 & $0.504^{+0.026}_{-0.032}$ & $0.402^{+0.025}_{-0.018}$ \\
NGC2360 & 421 & 0.444 & $0.085^{+0.055}_{-0.074}$ & $0.516^{+0.030}_{-0.036}$ \\
Stock2 & 410 & 0.802 & $0.779^{+0.021}_{-0.022}$ & $0.394^{+0.019}_{-0.016}$ \\
NGC2447 & 377 & 0.267 & $0.000^{+0.012}_{-0.000}$ & $0.375^{+0.011}_{-0.017}$ \\
\textbf{Hyades} & 369 & 0.424 & $0.209^{+0.054}_{-0.077}$ & $0.421^{+0.044}_{-0.028}$ \\
NGC2422 & 343 & 0.358 & $0.000^{+0.054}_{-0.000}$ & $0.457^{+0.008}_{-0.036}$ \\
NGC6281 & 309 & 0.546 & $0.510^{+0.020}_{-0.025}$ & $0.316^{+0.020}_{-0.016}$ \\
NGC0884 & 300 & 1.445 & $1.444^{+0.024}_{-0.024}$ & $0.419^{+0.019}_{-0.016}$ \\
IC4756 & 299 & 0.597 & $0.453^{+0.047}_{-0.062}$ & $0.473^{+0.043}_{-0.029}$ \\
NGC1039 & 296 & 0.400 & $0.000^{+0.050}_{-0.000}$ & $0.518^{+0.011}_{-0.037}$ \\
\textbf{alphaPer} & 284 & 0.736 & $0.284^{+0.110}_{-0.163}$ & $0.778^{+0.087}_{-0.052}$ \\
NGC2548 & 284 & 0.331 & $0.000^{+0.060}_{-0.000}$ & $0.421^{+0.006}_{-0.039}$ \\
NGC6405 & 275 & 0.688 & $0.578^{+0.043}_{-0.054}$ & $0.489^{+0.042}_{-0.029}$ \\
NGC0869 & 264 & 1.423 & $1.423^{+0.026}_{-0.027}$ & $0.424^{+0.020}_{-0.017}$ \\
IC4725 & 258 & 1.088 & $1.086^{+0.022}_{-0.022}$ & $0.356^{+0.018}_{-0.015}$ \\
NGC2423 & 255 & 0.474 & $0.118^{+0.067}_{-0.099}$ & $0.537^{+0.042}_{-0.043}$ \\
NGC6025 & 243 & 0.558 & $0.534^{+0.022}_{-0.023}$ & $0.296^{+0.020}_{-0.015}$ \\
\textbf{Blanco1} & 191 & 0.265 & $0.000^{+0.014}_{-0.000}$ & $0.422^{+0.020}_{-0.023}$ \\
NGC6633 & 190 & 0.562 & $0.478^{+0.041}_{-0.053}$ & $0.392^{+0.041}_{-0.027}$ \\
Trump10 & 175 & 0.428 & $0.000^{+0.029}_{-0.000}$ & $0.636^{+0.029}_{-0.040}$ \\
NGC7092 & 174 & 0.338 & $0.000^{+0.025}_{-0.000}$ & $0.497^{+0.023}_{-0.032}$ \\
\textbf{IC2602} & 173 & 0.805 & $0.000^{+0.203}_{-0.000}$ & $1.020^{+0.018}_{-0.127}$ \\
\textbf{NGC2451} & 145 & 0.747 & $0.000^{+0.146}_{-0.000}$ & $0.970^{+0.030}_{-0.104}$ \\
NGC2323 & 143 & 0.637 & $0.601^{+0.034}_{-0.042}$ & $0.357^{+0.036}_{-0.024}$ \\
NGC0752 & 141 & 0.408 & $0.000^{+0.039}_{-0.000}$ & $0.586^{+0.028}_{-0.044}$ \\
\textbf{IC2391} & 134 & 0.732 & $0.000^{+0.176}_{-0.000}$ & $0.938^{+0.024}_{-0.116}$ \\
Trump02 & 134 & 0.848 & $0.842^{+0.030}_{-0.032}$ & $0.339^{+0.026}_{-0.021}$ \\
NGC2158 & 132 & 1.107 & $1.078^{+0.050}_{-0.057}$ & $0.537^{+0.049}_{-0.035}$ \\
NGC6774 & 127 & 0.495 & $0.339^{+0.071}_{-0.115}$ & $0.424^{+0.076}_{-0.039}$ \\
NGC2547 & 122 & 0.729 & $0.000^{+0.088}_{-0.000}$ & $1.028^{+0.052}_{-0.086}$ \\
\textbf{ComaBer} & 109 & 0.257 & $0.000^{+0.025}_{-0.000}$ & $0.391^{+0.024}_{-0.030}$ \\
NGC6793 & 103 & 0.962 & $0.961^{+0.031}_{-0.031}$ & $0.310^{+0.026}_{-0.019}$ \\
NGC1901 & 71 & 0.407 & $0.000^{+0.086}_{-0.000}$ & $0.554^{+0.032}_{-0.068}$ \\
NGC2232 & 70 & 0.681 & $0.000^{+0.121}_{-0.000}$ & $0.967^{+0.064}_{-0.108}$ \\
Coll140 & 63 & 0.647 & $0.000^{+0.109}_{-0.000}$ & $0.956^{+0.072}_{-0.105}$ \\
NGC3228 & 60 & 0.469 & $0.000^{+0.137}_{-0.000}$ & $0.616^{+0.032}_{-0.095}$ \\
IC4665 & 56 & 0.691 & $0.666^{+0.052}_{-0.068}$ & $0.354^{+0.062}_{-0.034}$ \\
%
\hline
\end{tabular}
\end{center}
\end{table}


Finally, we can see from Table~\ref{table:cluster-extinction-estimates} that the maximum-likelihood estimates of $\sigma$ vary quite considerably, sometimes being below and sometimes above our global uncertainty estimate of 0.46\,mag from section~\ref{ssec:extinction-in-halo}. Unsurprisingly, the estimation of cluster extinctions works better for some samples than for others.

\message{ !name(cluster-ag-estimation.tex) !offset(-144) }

